Functionality learning through specification instructions

Test suites assess natural language processing models' performance on specific functionalities: cases of interest involving model robustness, fairness, or particular linguistic capabilities. This paper introduces specification instructions: text descriptions specifying fine-grained task-specific behaviors. For each functionality in a suite, we generate an instruction that describes it. We combine the specification instructions to create specification-augmented prompts, which we feed to language models pre-trained on natural instruction data. We conduct experiments to measure how optimizing for some functionalities may negatively impact functionalities that are not covered by the specification set. Our analyses across four tasks and models of diverse sizes and families show that smaller models struggle to follow specification instructions. However, larger models (>~3B params.) can benefit from specifications and -- surprisingly -- even generalize certain desirable behaviors across functionalities.

==> tables/qual_func.tex <==
\begin{table*}[tb]
    \scriptsize
    \centering
    \rowcolors{2}{gray!20}{white}
  \begin{tabularx}{\linewidth}{l>{\hsize=.45\hsize}X>{\hsize=.55\hsize}Xr}
    \toprule
    \rowcolor{white}
    Suite &Functionality &Example &$\Delta$ pass rate \\
    \midrule
    \texttt{SENT} &neutral words in context &That staff is Italian. &12.79 \\
    &Hard: Negation of negative with neutral stuff in the middle (should be positive or neutral) &i wouldn't say, given the time that I've been flying, that that is a ridiculous plane. &-12.30 \\
\midrule
\texttt{PARA} &Irrelevant preamble with different examples. &Q1: My pet monkey eats water. Is it normal for animals to eat water? \newline Q2: My pet lizard eats water. Is it normal for animals to eat water? &35.05 \\
&Simple coref: he and she &Q1: If Christopher and Erica were alone, do you think he would reject her? \newline Q2: If Christopher and Erica were alone, do you think she would reject him? &-37.37 \\
\midrule
\texttt{READ}  &Animal vs Vehicle v2 &C: Mark bought a duck. Danielle bought a truck. \newline Q: Who bought a vehicle? &31.45* \\
&Basic coref, he / she &C: Lisa and Cameron are friends. He is an adviser, and she is an author. \newline Q: Who is an adviser? &-18.86 \\
\midrule
\texttt{HATE} &threat\_dir\_h &I am going to make those disabled people suffer. &16.41 \\
&counter\_ref\_nh &It hurts to see all these people saying female lives are worthless. &-17.14 \\
\bottomrule
\end{tabularx}
\caption{Functionalities most harmed and helped by specification-augmented prompts. \newline *For \texttt{READ}, there was no functionality with positive pass rate difference when averaged across all models, so we show the difference when averaged only for ChatGPT.}
\label{tab:qualFunc}
\end{table*}
